Interactive Inverse Reinforcement Learning for Cooperative Games

We study the problem of designing autonomous agents that can learn to cooperate effectively with a potentially suboptimal partner while having no access to the joint reward function. This problem is modeled as a cooperative episodic two-agent Markov decision process. We assume control over only the first of the two agents in a Stackelberg formulation of the game, where the second agent is acting so as to maximise expected utility given the first agent's policy. How should the first agent act in order to learn the joint reward function as quickly as possible and so that the joint policy is as close to optimal as possible? We analyse how knowledge about the reward function can be gained in this interactive two-agent scenario. We show that when the learning agent's policies have a significant effect on the transition function, the reward function can be learned efficiently.

==> figures/figure_maze_maker_env/maze_maker.tex <==

\colorlet{DarkGreen}{green!60!black!40}
% FIRST
\begin{tikzpicture}[scale=0.74]

\fill[blue!5] (1.51, 1.51) -- +(0, .48) -- +(.48, .48) -- +(.48,0) -- cycle;
\draw[step=0.5cm,color=black!70] (0,0) grid (3.5,3.5);

\node at (1.75, 1.75) {\includegraphics[scale=0.05]{figures/mine-cart.png}};

\fill[DarkGreen!20] (0.51, 0.51) -- +(0, .48) -- +(.48, .48) -- +(.48,0) -- cycle;
\node at (0.75, 0.75) {\small +1};

\fill[DarkGreen!50] (3.01, 2.51) -- +(0, .48) -- +(.48, .48) -- +(.48,0) -- cycle;
\node at (3.25,2.75) {\small +2};

\fill[DarkGreen!90] (2.51, 0.01) -- +(0, .48) -- +(.48, .48) -- +(.48,0) -- cycle;
\node at (2.75, 0.25) {\small +3};
\end{tikzpicture}
\
% SECOND
\begin{tikzpicture}[scale=0.74]
\draw[step=0.5cm,color=black!70] (0,0) grid (3.5,3.5);
\fill[blue!5] (1.51, 1.51) -- +(0, .48) -- +(.48, .48) -- +(.48,0) -- cycle;

% % ARROWS
% North-East
\foreach \i/\j in {0/0, 1/4, 2/5, 3/0, 4/3, 6/5, 2/2, 3/2, 4/0}
{
    \draw[-to, black!70] (0.25 + \i *0.5, 0.25 +\j * 0.5) -- (0.25 + \i *0.5, 0.48 + \j *0.5);
    \draw[-to, black!70] (0.25 + \i *0.5, 0.25 +\j * 0.5) -- (0.48 + \i *0.5, 0.25 + \j *0.5);
}
% North-South
\foreach \i/\j in {0/1, 0/4, 1/0, 2/4, 5/0, 5/6}
{
    \draw[-to, black!70] (0.25 + \i *0.5, 0.25 +\j * 0.5) -- (0.25 + \i *0.5, 0.48 + \j *0.5);
    \draw[-to, black!70] (0.25 + \i *0.5, 0.25 +\j * 0.5) -- (0.25 + \i *0.5, 0.02 + \j *0.5);
}

% North-West
\foreach \i/\j in {6/0, 3/3, 2/3, 1/1, 3/1, 3/4, 3/6, 5/1, 5/2}
{
    \draw[-to, black!70] (0.25 + \i *0.5, 0.25 +\j * 0.5) -- (0.25 + \i *0.5, 0.48 + \j *0.5);
    \draw[-to, black!70] (0.25 + \i *0.5, 0.25 +\j * 0.5) -- (0.02 + \i *0.5, 0.25 + \j *0.5);
}

% South-East
\foreach \i/\j in {0/6, 1/3, 1/2, 2/0, 2/1, 4/1, 5/3, 5/4, 6/1, 6/2}
{
    \draw[-to, black!70] (0.25 + \i *0.5, 0.25 +\j * 0.5) -- (0.25 + \i *0.5, 0.02 + \j *0.5);
    \draw[-to, black!70] (0.25 + \i *0.5, 0.25 +\j * 0.5) -- (0.48 + \i *0.5, 0.25 + \j *0.5);
}

% South-West
\foreach \i/\j in {6/6, 0/2, 0/5, 2/6, 3/5, 4/2, 4/4}
{
    \draw[-to, black!70] (0.25 + \i *0.5, 0.25 +\j * 0.5) -- (0.25 + \i *0.5, 0.02 + \j *0.5);
    \draw[-to, black!70] (0.25 + \i *0.5, 0.25 +\j * 0.5) -- (0.02 + \i *0.5, 0.25 + \j *0.5);
}

% West-East
\foreach \i/\j in {0/3, 1/5, 1/6, 4/5, 4/6, 5/5, 6/3, 6/4}
{
    \draw[-to, black!70] (0.25 + \i *0.5, 0.25 +\j * 0.5) -- (0.02 + \i *0.5, 0.25 + \j *0.5);
    \draw[-to, black!70] (0.25 + \i *0.5, 0.25 +\j * 0.5) -- (0.48 + \i *0.5, 0.25 + \j *0.5);
}


\end{tikzpicture}
\
% THIRD
\begin{tikzpicture}[scale=0.74]
\fill[blue!5] (1.51, 1.51) -- +(0, .48) -- +(.48, .48) -- +(.48,0) -- cycle;
\draw[step=0.5cm,color=black!70] (0,0) grid (3.5,3.5);

\fill[DarkGreen!20] (0.51, 0.51) -- +(0, .48) -- +(.48, .48) -- +(.48,0) -- cycle;
\node at (2.25, 0.25) {\includegraphics[scale=0.05]{figures/mine-cart.png}};

\fill[DarkGreen!50] (3.01, 2.51) -- +(0, .48) -- +(.48, .48) -- +(.48,0) -- cycle;
\node at (3.25,2.75) {\small +2};

\fill[DarkGreen!90] (2.51, 0.01) -- +(0, .48) -- +(.48, .48) -- +(.48,0) -- cycle;
\node at (2.75, 0.25) {\small +3};

\draw[-, black!70] (0.25+3*0.5, 0.25+3*0.5) -- (0.25 + 1*0.5, 0.25 +3*0.5);
\draw[-, black!70] (0.25+1*0.5, 0.25+3*0.5) -- (0.25 + 1*0.5, 0.25 +1*0.5);
\draw[-, black!70] (0.25+1*0.5, 0.25+1*0.5) -- (0.25 + 2*0.5, 0.25 +1*0.5);
\draw[-, black!70] (0.25+2*0.5, 0.25+1*0.5) -- (0.25 + 2*0.5, 0.25 +0*0.5);
\draw[-to, black!70] (0.25+2*0.5, 0.25+0*0.5) -- (0.5 + 3*0.5, 0.25 +0*0.5);
\filldraw[black!70] (0.25+3*0.5, 0.25+3*0.5) circle (1pt);


\end{tikzpicture}


% \begin{tikzpicture}[scale=1]
% \draw[step=0.5cm,color=gray, thick] (0,0) grid (3.5,3.5);
% \fill[blue!5] (1.51, 1.51) -- +(0, .48) -- +(.48, .48) -- +(.48,0) -- cycle;
% \node at (1.75, 1.75) {\small $\A$};

% \fill[DarkGreen!20] (0.51, 0.51) -- +(0, .48) -- +(.48, .48) -- +(.48,0) -- cycle;
% \node at (0.75, 0.75) {\small +1};

% \fill[DarkGreen!50] (3.01, 2.51) -- +(0, .48) -- +(.48, .48) -- +(.48,0) -- cycle;
% \node at (3.25,2.75) {\small +2};

% \fill[DarkGreen!90] (2.51, 0.01) -- +(0, .48) -- +(.48, .48) -- +(.48,0) -- cycle;
% \node at (2.75, 0.25) {\small +3};
% \end{tikzpicture}
% \quad
% \begin{tikzpicture}[scale=1]
% \fill[blue!5] (1.51, 1.51) -- +(0, .48) -- +(.48, .48) -- +(.48,0) -- cycle;
% \draw[step=0.5cm,color=gray, thick] (0,0) grid (3.5,3.5);

% \fill[DarkGreen!20] (0.51, 0.51) -- +(0, .48) -- +(.48, .48) -- +(.48,0) -- cycle;
% \node at (0.75, 0.75) {\small $\A$};

% \fill[DarkGreen!50] (3.01, 2.51) -- +(0, .48) -- +(.48, .48) -- +(.48,0) -- cycle;
% \node at (3.25,2.75) {\small +2};

% \fill[DarkGreen!90] (2.51, 0.01) -- +(0, .48) -- +(.48, .48) -- +(.48,0) -- cycle;
% \node at (2.75, 0.25) {\small +3};
% \end{tikzpicture}

==> sections/acknoweldgements.tex <==
\section*{Acknowledgements}
This work was supported by the Norwegian Research Council through grant 302203.

==> sections/old_proofs.tex <==

\subsubsection{Proof of Lemma \ref{lemma:value_iteration_for_epsilon}}


For a policy $\pi^1$, we denote the space of optimal responses by $\optPi_2 (\pi^1)$ and let $\pi^*(\pi^1) \in \optPi_2(\pi^1)$ denote a fixed optimal response to $\pi^1$. An $\varepsilon$-greedy policy given $\pi^1$ is then defined as
\begin{align*}
    \pi^2_\varepsilon (s, \pi^1) =
    \begin{cases}
    \pi^*(s, \pi^1) & w.p.\ 1-\varepsilon \\
    \mathcal{U}(A_2) & w.p.\ \varepsilon,
    \end{cases}
\end{align*}
where $\varepsilon \in [0,1]$ and $\mathcal{U}(A_2)$ is the uniform distribution over $A_2$. We define the optimal value function $V^*$ as
\begin{align*}
    V^*(s) \defn \sup_{\pi^1} V_{\pi^1, \pi^2_\varepsilon(\pi^1)}(s) \quad \forall s \in \S,
\end{align*}
where we want to emphasise that the supremum is taken separably for each $s \in \S$. In particular, Theorem \ref{lemma:no_dominating_policy} tells us that for some classes of responses, e.g.\ $\bolPi_2$, there may not exists a policy $\pi^1$ such that $V_{\pi^1, \pi^2_\varepsilon(\pi^1)} (s) = V^*(s)$ for all $s \in \S$. 

The problem of planning with an agent that responds with $\varepsilon$-greedy policies is similar to the setting considered by \cite{dimitrakakis2017multi} in the sense that $\A_2$ plans with the original transition kernel $\trans$ (by computing $\pi^*(\pi^1)$), whereas $\A_1$ plans with the ``correct'' transition kernel
\begin{align*}
    \trans_\varepsilon(s' \mid s, a, b) \defn \varepsilon \trans (s' \mid s, a, \mathcal{U}(A_2)) + (1-\varepsilon) \trans (s' \mid s, a, b).
\end{align*} 
In particular, note that $\varepsilon \trans(s' \mid s, a, \mathcal{U}(A_2))$ is independent of the choice of $b$. 

We define the following two operators on the normed vector space $\mathcal{V} = \{ V: \S \to \Reals \colon \| V\|_{\infty} < \infty\}$ equipped with the supremum norm $\lVert \cdot \rVert_{\infty}$
\begin{align*}
    T_{\pi^1}V(s) & = \max_{b} \r(s) + \gamma \sum_{s'} \trans_{\varepsilon} (s' \mid s, \pi^1, b) V(s') \\
    %& = \varepsilon \big(\r(s) + \gamma \sum_{s'} \trans(s'\mid s, \pi^1, \mathcal{U}(A_2)) V(s') \big) + (1-\varepsilon) \max_b \big( \r(s) + \gamma \sum_{s'} \trans(s'\mid s, \pi^1, b) V(s')\big)
    T V(s) & = \max_a \max_b \r(s) + \gamma \sum_{s'} \trans_{\varepsilon} (s' \mid s, a, b) V(s').
\end{align*}
To show that a dominating commitment strategy always exists, we will need that $T_{\pi^1}$ and $T$ are $\gamma$-contractions w.r.t.\ $\lVert \cdot \rVert_{\infty}$. 

\begin{lemma}
The operator $T_{\pi^1}$ is a $\gamma$-contraction on $(\mathcal{V}, \lVert \cdot \rVert_{\infty})$ with unique fix point $V_{\pi^1, \pi^2_\varepsilon(\pi^1)}$. 
\end{lemma}
\begin{proof}
Note that for any two bounded functions $f, g: X \to \Reals$, the following standard inequality holds 
\begin{align}\label{equation:supremum_inequality}
    |\sup_{x \in X} f(x) - \sup_{x \in X} g(x)| \leq \sup_{x \in X} | f(x) - g(x) |.
\end{align}
For any $\pi^1$, we then obtain
\begin{align*}
    \lVert T_{\pi^1} V - T_{\pi^1} U \rVert_{\infty} & = \gamma \sup_{s} | \max_{b} \sum_{s'} \trans_{\varepsilon} (s' \mid s, \pi^1, b) V(s') - \max_{b} \sum_{s'} \trans_{\varepsilon} (s' \mid s, \pi^1, b) U(s') | \\
    & \overset{\eqref{equation:supremum_inequality}}{\leq} \gamma \sup_{s} \max_{b} | \sum_{s'} \trans_{\varepsilon} (s' \mid s, \pi^1, b) (V(s') - U(s'))|\\ 
    % & \leq \gamma \sup_{s} \max_b \sum_{s'} \trans_{\varepsilon} (s' \mid s, \pi^1, b) |V(s')- U(s')|  \\
    & \leq \gamma \sup_s \max_b \sum_{s'} \trans_{\varepsilon} (s' \mid s, \pi^1, b) \lVert V - U \rVert_{\infty} \\
    & = \gamma \lVert V - U \rVert_{\infty}.
\end{align*}
Thus, $T_{\pi^1}$ is a $\gamma$-contraction on $(\mathcal{V}, \lVert \cdot\rVert_{\infty})$. 
In the same vein, by applying equation \eqref{equation:supremum_inequality} to the maximisation $\max_{a} \max_{b}$, we get
\begin{align*}
    \lVert T V - T U \rVert_{\infty} & \leq \gamma \sup_s \max_a \max_b \sum_{s'} \trans_{\varepsilon} (s' \mid s, a, b) \lVert V- U\rVert_{\infty} = \gamma \lVert V - U \rVert_{\infty}.
\end{align*}
Hence, $T$ is a $\gamma$-contractions on $(\mathcal{V}, \lVert \cdot\rVert_{\infty})$. 
\end{proof}


\textcolor{purple}{Need to show that $V_{\pi^1, \pi^2_\varepsilon(\pi^1)}$ is a fix point of $T_{\pi^1}$}

\begin{proof}[\textbf{Proof of Lemma \ref{lemma:value_iteration_for_epsilon}}]
The following proof holds for a possibly infinite state space $\S$ and for finite actions spaces $A_1$ and $A_2$.\footnote{The extension to infinite actions spaces requires an additional continuity assumption to guarantee the existence of a greedy policy. (I think)} If not differently specified, let $s, s' \in \S$, $a \in A_1$ and $b \in A_2$. 





Let $s \in S$. By definition of $V^*$, we have $V_{\pi^1, \pi^2_\varepsilon(\pi^1)} (s) \leq V^*(s)$ for any $\pi^1$. Applying the operator $T_{\pi^1}$ on both sides, we then get $V_{\pi^1, \pi^2_\varepsilon(\pi^1)}(s) \leq T_{\pi^1} V^*$, where we have used that $\pi^1$ is the (unique) fix point of $T_{\pi^1}$. Taking the supremum over $\pi^1$ on both sides, it then follows that 
\begin{align*}
    V^*(s) = \sup_{\pi^1} V_{\pi^1, \pi^2_\varepsilon(\pi^1)} (s) \leq \sup_{\pi^1} T_{\pi^1} V^*(s) = TV^*(s),
\end{align*}
where the last equality holds by definition of $T_{\pi^1}$ and $T$. Crucially, note that taking the supremum over all $s \in \S$, i.e.\ $\sup_{\pi^1} V_{\pi^1, \pi^2_{\varepsilon}(\pi^1)}$, would not be well-defined as we do not know whether a dominating policy $\pi^1$ maximising $V_{\pi^1, \pi^2_{\varepsilon}(\pi^1)}(s)$ for all $s\in \S$ exists. However, we are can establish the above relation for each $s \in \S$ separably.

We now define the policy $\pi^1$ as the policy such that $T_{\pi^1}V^* = T V^*$, i.e.\ for $s \in \S$
\begin{align*}
    \pi^1(s) = \argmax_{a} \max_b \r(s) + \gamma \sum_{s'} \trans_{\varepsilon} (s' \mid s, a, b) V^*(s').
\end{align*}
Note that $\pi^1$ is well-defined. In particular, while the $\varepsilon$-greedy response $\pi^2_{\varepsilon}$ depends on the complete policy $\pi^1$, we defined the operators $T_{\pi^1}$ and $T$ such that $\A_2$'s response is expressed using the term $\max_b$.

It follows that $T_{\pi^1} V^* \succeq V^*$ 
\vspace{2cm}

\end{proof}








==> sections/planning.tex <==

\section{Planning with Suboptimal Partners}\label{section:planning}
% Planning with irrational partners 
In our Algorithm we compute and play optimal joint policy ...

Given a belief about the reward function, we want to derive a policy $\pi^1$ maximizing utility.\mgcomment{are we still in the partial information setting so? do you mean pure exploitation, when you speak of ``planning''?} We show that if $\A_2$ responds optimally, it is sufficient to find the optimal joint policy as it yields an optimal commitment strategy for $\A_1$. The proofs of the following results can be found in Appendix~\ref{appendix:proofs}.
\begin{lemma}\label{lemma:optimal_joint_policy_optimal}
Let $(\hat \pi^1, \hat\pi^2) \in \argmax_{\pi^1, \pi^2} V_{\pi^1, \pi^2}$ be an optimal joint policy. If $\beta \to \infty$, i.e.\ $\A_2$ responds optimally to the commitment of $\A_1$, then $V_{\hat \pi^1, \pi^2(\hat\pi^1)} = \max_{\pi^1} V_{\pi^1, \pi^2(\pi^1)} = \max_{\pi^1, \pi^2} V_{\pi^1, \pi^2}$.
\end{lemma}
We can therefore compute the optimal joint policy given a belief about the reward function, which can be done in polynomial time in the number of states and actions when modeling the problem as a single-agent MDP with action space $A_1 \times A_2$. [Another general case, where computing the optimal commitment strategy becomes easy is when $\A_2$ policy is independent of $\A_1$'s commitment, e.g.\ $\A_2$ always plays uniformly at random.]

When $\A_2$ responds with Boltzmann-rational policies, we see that this is not the case. In fact, we show that if $\A_2$ plays proportionally w.r.t.\ the expected value of taking an action, a dominating policy for $\A_1$ may fail to exist, i.e.\ there is no policy $\pi^1$ such that $V_{\pi^1, \pi^2(\pi^1)}(s) \geq V_{\hat \pi^1, \pi^2(\hat \pi^1)}(s)$ for all $\hat \pi^1$ and $s \in \S$. 


\begin{theorem}\label{lemma:no_dominating_policy}
If $\pi^2 (\actb \mid s) \propto f(Q_{\pi^1}^*(s, \actb))$ for any strictly increasing function $f:[0, \infty) \to [0, \infty)$, then a dominating commitment strategy for agent $\A_1$ may not exist.
\end{theorem}

In particular, this means that if $\A_2$ plays Boltzmann-rational, a dominating commitment strategy may fail to exist. 
Note that Theorem \ref{lemma:no_dominating_policy} generally only holds for {\em strictly} increasing functions $f$, as, for instance, there always exists a dominating commitment strategy when $\A_2$ plays uniformly at random. However, even for responses as simple as $\varepsilon$-greedy policies, we can show that a dominating commitment may fail to exist.

\begin{lemma}\label{lemma:eps_greedy_dominating}
If $\A_2$ plays $\varepsilon$-greedy responses, a dominating commitment strategy for $\A_1$ may not exist. 
\end{lemma}

We prove Theorem \ref{lemma:no_dominating_policy} and Lemma \ref{lemma:eps_greedy_dominating} by counterexample in Appendix X.

Note that the existence of a dominating policy is closely linked to our capacity to compute an optimal policy as it is fundamental requirement for dynamic programming. Despite this difficulty, we provide algorithms to approximately solve the problem of planning with suboptimal agents in Appendix X.


\iffalse
THIS IS FALSE
\begin{lemma}\label{lemma:value_iteration_for_epsilon}
If $\A_2$ responds with $\varepsilon$-greedy policies to $\A_1$'s commitment, then there always exists a dominating commitment strategy and a variant of the value iteration algorithm (see Algorithm A) converges to said commitment strategy. 
\end{lemma}
\fi




==> sections/zzz_changes.tex <==

\begin{algorithm}[tb]
    \caption{Interactive IRL via Linear Programming}
    \label{algorithm:full_info_opt_behaviour}
\begin{algorithmic}[1]
\STATE {\bfseries input:} $(\S, A_1, A_2, \trans, \gamma)$, initial policy $\pi^1_1$
\FOR{$t = 1, 2, \dots $}
\STATE commit to policy $\pi^1_t$ % and observe response $\pi^2_t$
\STATE observe response $\pi^2_t$
\STATE get constraints $\mathcal{C}_t = \mathcal{C}((\pi^1_1, \pi^2_1),\dots, (\pi^1_t, \pi^2_t))$
\STATE sample objective vector $c$ uniformly at random
\STATE find solution $R_t$ of LP with constraints $\mathcal{C}_t$ and objective $c$ 
\STATE compute optimal commitment strategy $\pi^1_{t+1}$ under $R_t$ 
\ENDFOR
\end{algorithmic}
\end{algorithm}

